Domain Adaptation for Dense Retrieval and Conversational Dense Retrieval through Self-Supervision by Meticulous Pseudo-Relevance Labeling

Recent studies have demonstrated that the ability of dense retrieval models to generalize to target domains with different distributions is limited, which contrasts with the results obtained with interaction-based models. Prior attempts to mitigate this challenge involved leveraging adversarial learning and query generation approaches, but both approaches nevertheless resulted in limited improvements. In this paper, we propose to combine the query-generation approach with a self-supervision approach in which pseudo-relevance labels are automatically generated on the target domain. To accomplish this, a T5-3B model is utilized for pseudo-positive labeling, and meticulous hard negatives are chosen. We also apply this strategy on conversational dense retrieval model for conversational search. A similar pseudo-labeling approach is used, but with the addition of a query-rewriting module to rewrite conversational queries for subsequent labeling. This proposed approach enables a model's domain adaptation with real queries and documents from the target dataset. Experiments on standard dense retrieval and conversational dense retrieval models both demonstrate improvements on baseline models when they are fine-tuned on the pseudo-relevance labeled data.

==> tables/bioasq.tex <==
\begin{tabular}{|c|c|}
\hline
model &  nDCG@10 (\%) \\
\hline
\multicolumn{2}{|c|}{\textit{Zero-Shot Models}} \\
\hline
D-BERT & 53.6 
\\
BM25 (Anserini) & 73.0\\
\hline
\multicolumn{2}{|c|}{\textit{Re-Ranking with Cross-Encoders (Upper Bound)}} \\ \hline
BM25 + CE   & 72.8\\
BM25 + T53B   & 76.1\\ \hline
\multicolumn{2}{|c|}{\textit{Previous Domain Adaptation Methods}} \\ \hline
UDALM                                      & 33.1 \\
MoDIR (ANCE) & 47.9\\
\hline
\multicolumn{2}{|c|}{\textit{Pre-Training based: Target $\to$ D-BERT}}                                       \\ 
\hline
SimCSE & 53.2 \\
ICT & 55.3 \\
TSDAE & 55.5 \\
\hline
\multicolumn{2}{|c|}{\textit{Generation-based (Previous SOTA)}} \\ 
\hline
QGen    & 56.5\\
GPL & 62.8
\\
TSDAE + GPL & 61.6\\
\hline

\multicolumn{2}{|c|}{Proposed: T53B, Global Random Neg}
  \\ 
\hline
DoDress-T53B (D-BERT) & 52.9


\\
DoDress-T53B (GPL) & 62.0


\\ \hline
\multicolumn{2}{|c|}{Proposed: T53B, BM25 Hard Neg}       \\ 
\hline
DoDress-BM25 (D-BERT) & 58.6

\\
DoDress-BM25 (GPL) & 64.7

\\
\hline
\multicolumn{2}{|c|}{Proposed: T53B, SimANS Hard Neg}
  \\ 
\hline
DoDress-T53B (D-BERT) & \textbf{60.6}

\\ 
DoDress-T53B (GPL) & \textbf{65.3}

\\ \hline
\end{tabular}

==> tables/robust.tex <==
\begin{tabular}{|c|c|}
\hline
model &  nDCG@10 (\%) \\
\hline
\multicolumn{2}{|c|}{\textit{Zero-Shot Models}} \\
\hline
D-BERT & 39.1 

\\
BM25 (Anserini) &  44.4\\
\hline
\multicolumn{2}{|c|}{\textit{Re-Ranking with Cross-Encoders (Upper Bound)}} \\ \hline
BM25 + CE   & 45.8\\
BM25 + T53B   & 51.8\\ \hline

\multicolumn{2}{|c|}{\textit{Generation-based (Previous SOTA)}} \\ 
\hline
GPL & 41.9

\\
TSDAE + GPL &  40.7

\\
\hline

\multicolumn{2}{|c|}{Proposed: T53B, Global Random Neg}
  \\ 
\hline
DoDress-T53B (D-BERT) &
40.5

\\
DoDress-T53B (GPL) & 
% 43.2
43.2
\\ \hline
\multicolumn{2}{|c|}{Proposed: T53B, BM25 Hard Neg}       \\ 
\hline
DoDress-BM25 (D-BERT) & 
% 41.1
41.6
\\
DoDress-BM25 (GPL) & 
% 43.0
43.3

\\
\hline
\multicolumn{2}{|c|}{Proposed: T53B, SimANS Hard Neg}
  \\ 
\hline
DoDress-T53B (D-BERT) & \textbf{43.6}

\\
DoDress-T53B (GPL) & \textbf{45.5}

\\ \hline
\end{tabular}
